Omnidirectional perfect acoustic cloak realized by homogeneous materials

Acoustic cloaks derived by coordinate transformation have opened up a new field of considerable interest in the last two decades. However, since perfect omnidirectional acoustic cloak relies on inhomogeneous and anisotropic materials that posses extreme values in certain regions, this cloak was deemed impossible to be attained even with metamaterials. Recently, our group was competent to introduce a new kind of extreme acoustic material, named as acoustic null medium (ANM), for attaining various devices. In this letter, an extreme mapping function is exploited to achieve an omnidirectional acoustic cloak. The attained extreme homogeneous material through this transformation becomes ANM that can satisfy the extreme parameters requirement and as a result, can hide the object from any incident acoustic waves. Several numerical simulations were carried out to demonstrate the capability of the propounded cloak in cloaking objects from sound fields. The propounded work will pave the way towards cloaking arbitrary objects from any incident angle and obviate the conventional challenges regarding this device.

==> Ref.tex <==
@article{pendry2006controlling,
	title={Controlling electromagnetic fields},
	author={Pendry, John B and Schurig, David and Smith, David R},
	journal={science},
	volume={312},
	number={5781},
	pages={1780--1782},
	year={2006},
	publisher={American Association for the Advancement of Science}
}
@article{fakheri2017carpet,
	title={Carpet cloak design for rough surfaces},
	author={Fakheri, Mohammad Hosein and Barati, Hooman and Abdolali, Ali},
	journal={Chinese Physics Letters},
	volume={34},
	number={8},
	pages={084101},
	year={2017},
	publisher={IOP Publishing}
}

@article{chen2010acoustic,
	title={Acoustic cloaking and transformation acoustics},
	author={Chen, Huanyang and Chan, Che Ting},
	journal={Journal of Physics D: Applied Physics},
	volume={43},
	number={11},
	pages={113001},
	year={2010},
	publisher={IOP Publishing}
}

@article{cummer2007one,
	title={One path to acoustic cloaking},
	author={Cummer, Steven A and Schurig, David},
	journal={New Journal of Physics},
	volume={9},
	number={3},
	pages={45},
	year={2007},
	publisher={IOP Publishing}
}
%%%%%

@article{li2008hiding,
	title={Hiding under the carpet: a new strategy for cloaking},
	author={Li, Jensen and Pendry, John B},
	journal={Physical review letters},
	volume={101},
	number={20},
	pages={203901},
	year={2008},
	publisher={APS}
}


@article{ma2009compact,
	title={Compact-sized and broadband carpet cloak and free-space cloak},
	author={Ma, Hui Feng and Jiang, Wei Xiang and Yang, Xin Mi and Zhou, Xiao Yang and Cui, Tie Jun},
	journal={Optics Express},
	volume={17},
	number={22},
	pages={19947--19959},
	year={2009},
	publisher={Optical Society of America}
}

@article{kallos2009ground,
	title={Ground-plane quasicloaking for free space},
	author={Kallos, Efthymios and Argyropoulos, Christos and Hao, Yang},
	journal={Physical Review A},
	volume={79},
	number={6},
	pages={063825},
	year={2009},
	publisher={APS}
}

@article{ma2010three,
	title={Three-dimensional broadband ground-plane cloak made of metamaterials},
	author={Ma, Hui Feng and Cui, Tie Jun},
	journal={Nature communications},
	volume={1},
	pages={21},
	year={2010},
	publisher={Nature Publishing Group}
}

%%%

@article{xi2009one,
	title={One-directional perfect cloak created with homogeneous material},
	author={Xi, Sheng and Chen, Hongsheng and Wu, Bae-Ian and Kong, Jin Au},
	journal={IEEE Microwave and Wireless Components Letters},
	volume={19},
	number={3},
	pages={131--133},
	year={2009},
	publisher={IEEE}
}

@article{landy2013full,
	title={A full-parameter unidirectional metamaterial cloak for microwaves},
	author={Landy, Nathan and Smith, David R},
	journal={Nature materials},
	volume={12},
	number={1},
	pages={25},
	year={2013},
	publisher={Nature Publishing Group}
}
@article{zhang2010lateral,
	title={Lateral shift makes a ground-plane cloak detectable},
	author={Zhang, Baile and Chan, Tucker and Wu, Bae-Ian},
	journal={Physical review letters},
	volume={104},
	number={23},
	pages={233903},
	year={2010},
	publisher={APS}
}
%%%%

@article{fakheri2018arbitrary,
	title={Arbitrary Shaped Acoustic Concentrators Enabled by Nihility Media},
	author={Fakheri, Mohammad Hosein and Sedeh, Hooman Barati and Abdolali, Ali},
	journal={arXiv preprint arXiv:1812.07442},
	year={2018}
}
@article{sun2019full,
	title={Full space destructive interference by acoustic-null medium},
	author={Sun, Fei and Liu, Yichao and Yang, Yibiao and Chen, Zhihui and He, Sailing},
	journal={Applied Physics Express},
	year={2019},
	publisher={IOP Publishing}
}

@article{li2017acoustic,
	title={Acoustic surface transformation realized by acoustic-null materials using bilayer natural materials},
	author={Li, Borui and Sun, Fei and He, Sailing},
	journal={Applied Physics Express},
	volume={10},
	number={11},
	pages={114001},
	year={2017},
	publisher={IOP Publishing}
}


@article{chen2007acoustic,
	title={Acoustic cloaking in three dimensions using acoustic metamaterials},
	author={Chen, Huanyang and Chan, CT},
	journal={Applied physics letters},
	volume={91},
	number={18},
	pages={183518},
	year={2007},
	publisher={AIP}
}


@article{li2004double,
	title={Double-negative acoustic metamaterial},
	author={Li, Jensen and Chan, Che Ting},
	journal={Physical Review E},
	volume={70},
	number={5},
	pages={055602},
	year={2004},
	publisher={APS}
}
